Human-in-the-Loop Imitation Learning using Remote Teleoperation

Imitation Learning is a promising paradigm for learning complex robot manipulation skills by reproducing behavior from human demonstrations. However, manipulation tasks often contain bottleneck regions that require a sequence of precise actions to make meaningful progress, such as a robot inserting a pod into a coffee machine to make coffee. Trained policies can fail in these regions because small deviations in actions can lead the policy into states not covered by the demonstrations. Intervention-based policy learning is an alternative that can address this issue -- it allows human operators to monitor trained policies and take over control when they encounter failures. In this paper, we build a data collection system tailored to 6-DoF manipulation settings, that enables remote human operators to monitor and intervene on trained policies. We develop a simple and effective algorithm to train the policy iteratively on new data collected by the system that encourages the policy to learn how to traverse bottlenecks through the interventions. We demonstrate that agents trained on data collected by our intervention-based system and algorithm outperform agents trained on an equivalent number of samples collected by non-interventional demonstrators, and further show that our method outperforms multiple state-of-the-art baselines for learning from the human interventions on a challenging robot threading task and a coffee making task. Additional results and videos at https://sites.google.com/stanford.edu/iwr .

==> 1-intro-v2.tex <==
\section{Introduction}
\label{sec:intro}

% Options (NOTE: currently going with 1)
% (1) talk about more general HITL setup, and then say that this won't work out of the box with human data on complex tasks, so we need to adapt HITL to work on complex tasks.
% (2) imitation learning is great, but humans are far from optimal for high-precision tasks. In these settings, it is natural to focus on important task-critical states, and a natural way is to allow for HITL to collect data on policy mistakes, but humans will still not have optimal interventions.

Imitation Learning (IL) is a promising paradigm for building complex manipulation skills by reproducing behaviors from human demonstrations~\cite{pomerleau1989alvinn, zhang2017deep, mandlekar2020learning}. Unlike interactive learning techniques, such as reinforcement learning, which generate large amounts of training data via autonomous exploration, the efficacy of IL is bounded by the cost of expert demonstrations. This cost limits the amount of data and the coverage of the state space with demonstrations available for training IL models. For this reason, models trained by IL can suffer from covariate shift: small errors in actions can bring the learner to non-annotated states that the learner has not been trained for. To address this covariate shift problem, DAgger-style methods~\cite{ross2011reduction,laskey2016shiv,kelly2019hg} iteratively collect additional data from the trained agent, relabeling the data using an expert, adding the relabeled data to the demonstration dataset and then re-training the agent. These methods allow for collecting training data on samples that the agent is likely to encounter. 
% Importantly, the data is relabeled by the expert in hindsight\roberto{the hindsight concept is not very clear. what is new to what you said before?}: for each state that was encountered by the agent, the expert must produce the action that they would have taken. 

% For real-world robotic tasks, however, DAgger-style data relabeling is often impractical, as it requires human demonstrators to provide corrective actions to all\roberto{right?otherwise what is the difference to intervention?} high-frequency control actions without gaining full control of the system \roberto{the full control thing is not clear}. 
For real-world robotic tasks, however, DAgger-style data relabeling is often impractical, as it requires human demonstrators to annotate high-frequency data samples that have already been collected by the agent with the actions that the human would have taken in those situations.
As a result, it requires significant human effort and is prone to incorrect action labels~\cite{laskey2017comparing}.
Instead, it is more natural for humans to annotate actions by directly controlling the robot.
% this process is infeasible for human demonstrators because it requires significant effort to relabel high-frequency manipulation data and can often result in incorrect labels~\cite{laskey2017comparing}. 
Consequently, in order to extend DAgger to real systems, prior work has proposed learning from active human interventions~\cite{kelly2019hg, spencerlearning, ablett2020fighting}. In these cases, the human demonstrator observes the robot performing a task and takes over control in regions where the robot is performing poorly, to provide new action labels.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/pullfig4.png}
    \caption{\textbf{Interactive Policy Learning with Human Interventions.} Manipulation tasks often contain bottleneck regions that require a series of precise actions to traverse successfully. Models trained on an offline set of human demonstrations easily fail in these regions due to action errors that compound. To address this issue, we built a system where a human operator observes a policy attempting to solve a manipulation task and intervenes when necessary to help solve the task. During an intervention, the human operator takes control of the arm from the policy, moves the robot arm into a state where the policy is likely to succeed, and then returns control to the policy. All data is aggregated into a dataset and the policy is re-trained on the new collected data. This process repeats. 
    }
    \label{fig:pull}
    \vspace{-15pt}
\end{figure}

% Interventions have been used mostly for driving domains, but manipulation can be more challenging. Former is very tolerant because there's lots of room of error in the "good" region of the state space to complete the task and only a few ways to fail. By contrast, manipulation requires structured set of actions to succeed, and is often not tolerant to error.

Learning from human interventions has been shown to be effective in driving domains~\cite{kelly2019hg, spencerlearning} while retaining the theoretical guarantees that DAgger provides on addressing covariate shift~\cite{spencerlearning}. 
In driving domains, the vehicle is typically tolerant to small errors over a period of time, such as wheel offsets, and these errors can be easily fixed by the human demonstrator with corrective steering actions.
% By contrast, robot manipulation, especially contact-rich tasks, often requires extended, fine-grained actions to complete the task successfully. In comparison to driving, the robot has many ways to fail in a manipulation task, but only a few ways to succeed.

% human interventions are particularly effective at demonstrating how to recover from unsafe regions and avoid revisiting them~\cite{spencerlearning}. However, the other regions of the state space are tolerant to a wide array of robot actions, since the robot must simply stay on track. In essence, there are many ways for the robot to succeed, but only a few ways for the robot to fail. 

Our key insight is that in contact-rich manipulation, there exists a set of \emph{task bottleneck}s -- regions that requires a precise sequence of actions to traverse in order to complete the task. For example, consider the peg insertion task shown in Fig.~\ref{fig:pull}. To complete the task, the robot must carefully insert the peg into the hole. This means that there is a very narrow set of locations in the state space that the robot must traverse.
% Example - insertion task has bottleneck, and it is easy for the agent to fail, so intervention-based learning is good here. There are many locations for the agent to fail.
Tasks with such bottlenecks are ideal testbeds for intervention-based learning, because covariate shift makes a robot trained from offline demonstrations susceptible to making mistakes in these regions. During insertion, the robot can easily find itself in states where the peg is misaligned with the hole, or where the peg misses the hole completely. By allowing a human to actively intervene when these task bottlenecks are encountered and demonstrate corrective behaviors, the robot will learn how to traverse the task bottlenecks from a wide array of states.

Making human interventions feasible for robot manipulation raises technical challenges on the system side as well as on the algorithmic side. First, we need a robust system that enables human demonstrators to monitor the robot behaviors with minimum location/time constraints and to gain immediate full control of the robot when observing imminent risks. Second, we need an effective algorithm that learns from mixed training data of human intervention samples and robot autonomous execution samples. To this end, we develop a system suitable for collecting intervention data from remote users with 6-DoF control of robot end-effectors and a simple yet effective method to leverage the human interventions in a way that pays special attention to bottleneck traversal by performing weighted regression.

The key intuition behind our algorithm is that in manipulation tasks, humans are likely to intervene when the robot has difficulty traversing bottlenecks, and to return control to the robot after traversing the bottleneck. Therefore, the human interventions are informative about both \textit{where} task bottlenecks occur and \textit{how} to traverse them. Our method leverages the signal of when the interventions are taking place for policy learning. We find that treating the intervention signal as an implicit reward function and performing weighted regression is highly effective.


% Leveraging the "task bottleneck" structure of the manipulation task can lead to substantial gains in intervention-based training in these domains. Because task bottlenecks require precise actions to traverse, human interventions are most likely to occur in the neighborhood of task bottlenecks. 
% While it is possible to directly learn from only the intervention samples collected by the human, 

%  In order to properly leverage that information, our method simultaneously leverages . 
 
%  We find that treating  in this setting. 

% In this paper, we address the problem of using human interventions to solve robot manipulation tasks. 

% Moreover, we expect the supervision to be consistent, because there are a small number of admissible states after traversing the bottleneck, compared to the rest of the state space. 
% To leverage this insight, 

\noindent \textbf{Summary of Contributions:}
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    leftmargin=*,
    itemindent=12pt]
\item We develop a system that enables remote teleoperation for 6-DoF robot control and a natural human intervention mechanism well suited to contact-rich manipulation.
\item We introduce \algoFull (\algoName) a simple yet effective method to learn from human interventions by guiding the policy to traverse bottleneck states.
\item We demonstrate that models trained on data collected by our human-in-the-loop system outperform models trained solely on same amounts of offline human demonstrations.
\item We show that our method consistently outperforms baselines over datasets collected from diverse human operators. We further demonstrate that our method can learn jointly from the multimodal data collected by all operators, where baselines fail to deal with conflicting supervision.
\end{enumerate}


==> 1-intro.tex <==
\section{Introduction}
\label{sec:intro}

% Options (NOTE: currently going with 1)
% (1) talk about more general HITL setup, and then say that this won't work out of the box with human data on complex tasks, so we need to adapt HITL to work on complex tasks.
% (2) imitation learning is great, but humans are far from optimal for high-precision tasks. In these settings, it is natural to focus on important task-critical states, and a natural way is to allow for HITL to collect data on policy mistakes, but humans will still not have optimal interventions.

Imitation Learning is a promising paradigm for learning complex robot manipulation skills by reproducing behavior from human demonstrations~\cite{pomerleau1989alvinn, zhang2017deep, mandlekar2020learning}. However, different to other learning techniques that can collect large amounts of data via autonomous exploration, IL is bounded by the burden of requesting expert humans to provide demonstrations. This limits the amount of data and the coverage of the state space with demonstrations typically available for IL. Due to the limited amount of data, IL policies can suffer from covariate shift: the distribution of learner actions diverges from the distribution of expert actions, taking the learner to explore non-annotated areas of the state space for which the learner has not been trained. DAgger-style methods~\cite{ross2011reduction} address this covariate shift problem by iteratively collecting additional data from the trained agent, relabeling the data using an expert, adding the data to the demonstration dataset and then re-training the agent. This allows for collecting training data on samples that the agent is actually likely to encounter. Importantly, the data is relabeled by the expert in hindsight - for each state that was encountered by the agent, the expert must produce the action that they would have taken. 

Unfortunately, for most realistic manipulation tasks this process is infeasible for human demonstrators because it requires a significant effort relabel high-frequency manipulation data and can often result in incorrect labels~\cite{laskey2017comparing}. In order to extend DAgger to human supervision, prior work has proposed learning from human interventions, where the human demonstrator observes the robot performing a task, and then takes over control in regions where the robot is performing poorly~\cite{kelly2019hg, spencerlearning, ablett2020fighting}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/placeholder.png}
    \caption{\textbf{Task Bottlenecks and Human Interventions:} Manipulation tasks often contain bottleneck regions that require a series of precise actions to traverse successfully. Agents trained on an offline set of human demonstrations easily fail in these regions due to action errors that compound (left). Allowing a human to intervene and provide data on how to traverse these bottlenecks can mitigate these issues. We build a data collection system and algorithm to collect and leverage such data (right).
    % The task is well-suited for intervention-based learning since human operators can demonstrate how to traverse the bottleneck when the robot, trained on an offline set of human demonstrations, makes mistakes. However, human interventions can be \textit{suboptimal} and \textit{multimodal} - for example, the human might take multiple attempts to do insertion, and the human could choose to intervene at different times.
    }
    \label{fig:pull}
    \vspace{-15pt}
\end{figure}

Learning from human interventions has been shown to be particularly effective in driving domains~\cite{kelly2019hg, spencerlearning} while retaining the same theoretical guarantees that DAgger provides for addressing covariate shift~\cite{spencerlearning}. However, prior approaches make the assumption that the human provides supervision that is optimal, or at the very least consistent and sufficient for task completion. This assumption is easily violated in robot manipulation settings that require extended, fine-grained actions to accomplish the task successfully.

For example, consider the insertion task shown in Fig.X. To complete the task, the robot must carefully insert the peg into the hole - this means that there is a very narrow set of locations in the state space that the robot must traverse. These locations form a \textit{task bottleneck} - a region that requires a precise sequence of actions to traverse in order to complete the task. Tasks with such bottlenecks are ideal for intervention-based data collection, because covariate shift makes it easy for a robot trained from offline demonstrations to make mistakes in these regions. However, a human supervisor that intervenes and takes control of the robot can also easily make mistakes due to the precision needed for traversing the bottleneck, and could take more than one attempt to guide the robot through the insertion. The human supervisor could also be inconsistent in when they choose to intervene and take control from the robot. This makes human supervision differ from an expert in two critical ways - the supervision is \textit{suboptimal}, taking longer than necessary to complete the task, and \textit{multimodal}, since there can easily be conflicting supervision at the same location. 

In this paper, we address the problem of using human interventions to solve high-precision robot manipulation tasks. Our key insight is that the human is likely to intervene when the robot has difficulty traversing task bottlenecks, and will return control to the robot after traversing the task bottleneck. The human supervision might be low-quality near the beginning of the intervention sequence due to the aforementioned reasons, but we expect the supervision at the end of the sequence to be high-quality, because it demonstrates how to traverse the bottleneck. Moreover, we expect the supervision to be consistent, because there are a small number of admissible states after traversing the bottleneck, compared to the rest of the state space.

To leverage this insight, we develop a system suitable for collecting intervention data in this setting and a simple and effective method to leverage the human interventions in a way that pays special attention to bottleneck traversal by weighting the loss of samples at the end of intervention segments.

\noindent \textbf{Summary of Contributions:}
\begin{enumerate}[
    topsep=0pt,
    noitemsep,
    leftmargin=*,
    itemindent=12pt]
\item We present a system that enables human-in-the-loop data collection for 6-DoF robot manipulation tasks and a natural human intervention mechanism that is well suited to high-precision manipulation.
\item We introduce a simple and effective method to learn from low-quality human interventions in this setting that encourages the agent to learn how to properly traverse bottleneck states in high-precision manipulation settings.
\item We demonstrate that agents trained on data collected by our intervention-based system outperform agents trained on an equivalent number of human-only demonstration samples, and that our method is able to better leverage the intervention data than alternatives.
\item We show that our method consistently outperforms baselines over datasets collected by multiple human operators, despite significant differences in the supervision provided by the operators. We further demonstrate that our method can learn jointly from the data collected by all operators, compared to baselines that are unable to deal with conflicting supervision.
\end{enumerate}


==> 2-related.tex <==
\section{Related Work}
\label{sec:related}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/sys_fig_v4.jpg}
    \caption{\textbf{System Overview.} We extend the RoboTurk system~\cite{mandlekar2018roboturk, mandlekar2019scaling} to enable remote users to monitor policy execution and intervene when they would like to take over control using a web browser and a smartphone. The user monitors policy execution by watching a video stream of the robot in their web browser. They can hold a button on their smartphone to intervene and control the robot by moving their smartphone.}
    \label{fig:system}
    % \vspace{0.5mm}
    \vspace{-15pt}
\end{figure}

\textbf{Imitation Learning from Offline Demonstrations:} Imitation learning can be used to train a policy from a set of offline expert demonstrations. A policy can be learned without any interaction, as in Behavioral Cloning (BC)~\cite{pomerleau1989alvinn, zhang2017deep, mandlekar2020learning} or using additional interaction with the environment, as in Inverse Reinforcement Learning (IRL)~\cite{abbeel2004apprenticeship, abbeel2011inverse}. However, policies trained with BC can suffer from \textit{covariate shift} because they are trained completely offline~\cite{ross2011reduction} -- it can be easy for the policy to encounter unseen states during evaluation. Because of this problem, BC often takes a prohibitive number of expert samples to work well. By contrast, IRL generally requires fewer expert samples, but it reply on a prohibitive amount of agent interaction with the environment~\cite{ho2016generative, zhu2018reinforcement, xu2019positive} due to the need to do reinforcement learning with a learned reward function. We instead focus on human-in-the-loop policy learning, which can strike a better balance between the number of human samples and agent samples required for learning.

% IRL can address this issue by learning a reward function that is consistent with the demonstration data and then training a policy in the environment to maximize the learned reward function.

% Some approaches also assume access to a reward function and train the policy in an offline~\cite{levine2020offline, fujimoto2018off, kumar2019stabilizing, mandlekar2020iris} or online~\cite{fan2018surreal, mandlekar2020learning, nair2018overcoming, vecerik2017leveraging} manner, leveraging the demonstration data in conjunction with the reward function. However, access to a reward function can be a large assumption in realistic settings. 

\textbf{Human-in-the-Loop Policy Learning:} Human-in-the-Loop Policy Learning allows the human to provide additional supervision during the policy learning process. One paradigm is Reinforcement Learning (RL) with human feedback~\cite{zhang2019leveraging}. Some methods have the human provide rewards while monitoring the agent~\cite{loftin2016learning, macglashan2017interactive, cabi2019scaling}, or discriminate between successful and unsuccessful outcomes produced by the agent~\cite{christiano2017deep, singh2019end, reddy2019learning}, allowing the agent to learn via RL from the human-provided labels. Human feedback has also been used to ensure safe exploration during RL~\cite{saunders2017trial}. These methods all suffer from the same drawbacks as IRL due to the need for extensive agent interaction while our method is sample efficient in both the number of agent samples and the number of human samples required. Other paradigms for human-in-the-loop policy learning include collaboration~\cite{hadfield2016cooperative, fisac2020pragmatic}, teaching the robot through informative sample selection~\cite{cakmak2012algorithmic, ho2016showing, brown2019machine}, and leveraging physical kinesthetic corrections~\cite{bajcsy2017learning, bajcsy2018learning}.

\textsc{DAgger}~\cite{ross2011reduction} introduced a useful paradigm for reducing the number of human samples needed for IL without performing explicit reinforcement learning. \textsc{DAgger} iteratively collects a set of samples with a trained policy, asks an expert to annotate these samples in hindsight with the actions that they would have taken, and then updates the policy by training with BC on the new data. 
\textsc{DAgger}~\cite{ross2011reduction} can require fewer expert samples than BC and fewer agent samples than IRL to train a policy.  However, \textsc{DAgger} is not feasible for humans in practical scenarios (e.g. continuous 6D control) due to the relabeling procedure, which can be burdensome and prone to human error, especially in manipulation settings~\cite{laskey2017comparing}. Prior work has attempted to reduce the number of human annotations needed~\cite{chernova2009interactive, laskey2016shiv, packard2017policies} but relabeling is still required. Noise injection during expert demonstrations has also been proposed in order to correct for covariate shift~\cite{laskey2017dart}. % In order to address the difficulty of human relabeling in \text{DAgger}, Kelly et al.~\cite{kelly2019hg} introduced \textsc{HG-DAgger}, a paradigm where human operators are able to take over control from an agent and demonstrate parts of a task that are difficult for the agent. 
% Other works have applied the paradigm in conjunction with active learning to query a human for interventions~\cite{ablett2020fighting}, and shown improved performance by learning from the timing of interventions~\cite{spencerlearning}. 

\textbf{Learning from Interventions:} In this work, we build a system that allows remote users to monitor policy execution and provide interventions, and a method that learns from the interventions intelligently. While similar systems have been built recently~\cite{ablett2020fighting, delpreto2020helping}, our system is the only one allowing for remote web-based operation and the only one demonstrated on contact-rich manipulation tasks.

Our method differs from prior intervention-based approaches~\cite{kelly2019hg, ablett2020fighting} by leveraging both human intervention samples, and agent samples leading to those interventions. While~\cite{spencerlearning} also uses intervention timings to favor some samples over others, their framework only applies to discrete action spaces, and uses the timings to penalize samples at the beginning of the intervention, treating all other samples equally. While this is suitable for driving domains, manipulation often has a large space of poor quality states (there are many ways to fail at insertion) and requires a precise sequence of actions to reach favorable states. We leverage intervention timings to prioritize the intervention samples over the rest of the data, encouraging the agent to learn how to traverse task bottlenecks while regularizing the behavior to that demonstrated by the current policy iterate. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/method_v3.png}
    \caption{\textbf{\algoFull.} Every intervention trajectory (blue box) consists of portions where the policy was controlling the robot (green) and portions where the human was intervening (red). These are aggregated to separate datasets. The intervention portions usually start in the neighborhood of bottlenecks that require a structured sequence of actions to traverse successfully and they demonstrate how to traverse them. During training (orange box), we sample equal size batches from the non-intervention and intervention datasets and train with a behavioral cloning loss. Sampling equal size batches from each dataset re-weights the data distribution to reinforce intervention actions that demonstrate bottleneck traversal, while the non-intervention samples provide regularization that keeps the policy close to previous policy iterates.}
    \label{fig:method_overview}
    % \vspace{0.5mm}
    \vspace{-15pt}
\end{figure}

% Our method differs from prior intervention-based approaches~\cite{kelly2019hg, ablett2020fighting} by leveraging both the human intervention samples, and the agent samples leading to those interventions. While~\cite{spencerlearning} also uses the timing of the interventions to favor some samples over others, their framework only applies to tasks with discrete action spaces and has only been demonstrated for driving tasks. By contrast, our framework addresses continuous control.



==> 5-experiment-v2.tex <==
\section{Experimental Setup}
\label{sec:exp}

\subsection{Tasks}
All tasks were designed using MuJoCo~\cite{todorov2012mujoco} and the robosuite framework~\cite{robosuite2020}. The workspace consists of a Sawyer robotic arm in front of a table. The arm is controlled using an Operational Space Controller~\cite{khatib1987unified} and unless otherwise mentioned, the action space for the agent is a 7-dimensional vector where the first 3 coordinates are the desired delta position from the current end effector position, the next 3 coordinates encode the desired delta rotation from the current end effector rotation, and the final coordinate controls the opening and closing of the gripper fingers. The delta rotation is encoded in axis-angle form, where the norm of the 3-vector is the angle, and normalizing the 3-vector produces the axis of the rotation.

\textbf{Threading}: At the start of each episode, a wooden rod  and wooden ring are placed on the table. The robot arm must pick up the wooden rod and insert it into the wooden ring. The location of the wooden rod and ring are randomized at the start of each episode. The insertion part of this task is significantly more challenging than the Peg-In-Hole task - insertion requires high precision, and it is easy for the robot arm to unintentionally move the wooden ring if the rod hits the ring. This task contains two bottleneck regions - the grasping of the rod and the insertion into the ring. The observation space consists of the end effector pose, gripper finger positions, and the poses of the wooden rod and ring.

\textbf{Coffee Machine}: At the start of each episode, a coffee pod and a coffee machine are placed on the table. The robot arm must pick up the coffee pod, insert it into the pod holder, and then close the lid of the coffee machine. The location of the coffee pod is randomized at the start of each episode. This task has three bottleneck regions - grasping, insertion, and closing. Both the pod grasping and insertion must be precise, as small errors will cause the pod to slip out of the hand, or fail to be inserted into the holder. The closing of the lid also requires extended contact between the lid and the hand, and misalignment in the closing motion would result in the lid staying open. The observation space consists of the end effector pose, gripper finger positions, the poses of the pod and pod holder, the hinge angle of the lid, and binary contact indicators between the pod, pod holder, and gripper fingers.

\subsection{Baselines}

In this section, we list the baselines we compare against and why each is meaningful.

\textbf{Human-Only}: A human operator collects full task demonstrations instead of intervention-based collection. The full trajectories are added to the dataset and policies are trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of leveraging intervention-based data collection tailored to policy failures over soliciting full task demonstrations that are agnostic to how policies fail on the task.

\textbf{HG-Dagger}: As in~\cite{kelly2019hg, ablett2020fighting} at each round of intervention data collection, only the samples where the user was intervening are added to the dataset, while the policy samples are discarded. Policies are trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of keeping policy samples to train the policy for the next round.

\textbf{Ours (no balancing)}: At each round of intervention data collection, all samples are added to the dataset, including the policy samples, and the next policy is trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of using balanced sampling in our method to reweight the data distribution.

\textbf{Ours}: Same as Ours (no balancing), but aggregates the policy samples and intervention samples into separate datasets and uses balanced sampling to re-weight the data distribution during learning.

\subsection{Experiment Details}

We conducted two data collection studies to demonstrate the utility of our system and our method for learning from intervention data. In the first, a single operator collected multiple sequences of datasets on the Threading and Coffee Machine tasks. In the second, multiple human operators collected datasets on the Coffee Machine tasks. 

% which amounted to 7205 samples for the Threading task, and 6620 samples for the Coffee Machine task
Each operator started with an initial dataset that consisted of 30 demonstrations for each task, and a base policy that was trained on each initial dataset. Then, for each intervention-based method, the operator performed 3 additional rounds of data collection. During each round, the operator collected trajectories until the number of intervention data samples reached roughly $33\%$ of the initial dataset samples. We only counted intervention data samples so that all methods would be able to receive the same number of human-annotated samples at each round, regardless of the quality of the base policy, and to be consistent with prior work~\cite{kelly2019hg}. After each round, the base policy for the next round was obtained by training for 2000 epochs on the aggregated dataset and taking the final checkpoint, in order to model the realistic setting where policy evaluation is expensive. Note that the Round 1 datasets will be the same for all methods but Round 2 and Round 3 will be different because data collection occurs on separate base policies.

For the "Human-Only" baseline, each operator collected a single dataset of human demonstration trajectories that consisted of roughly the same number of samples as the initial dataset. For the "Single" variants of the intervention-based methods, an operator performed a single round of intervention data collection on the initial base policy, gathering roughly the same number of intervention samples as the initial dataset. This dataset is shared for all methods for the same reason that the Round 1 datasets are the same.

All policies were Recurrent Neural Networks - 2-layer LSTMs with hidden dimension 100, trained on a sequence length of 10 using Adam optimizers~\cite{kingma2014adam}. To evaluate each method, policies were saved after every 50 epochs and evaluated with 50 rollouts for each checkpoint. All success rates presented in each table reflect the maximum average success rate obtained by each training run over all model checkpoints, for 3 training runs with different seeds. The procedure of training multiple runs, checkpointing, and evaluating policies was performed after data collection for all runs was complete - the numbers played no role in selecting base policies for the next round.

\subsection{Experiments}

\textbf{Does data collected using our intervention-based system improve task performance more than an equivalent amount of human-only demonstration samples?} To answer this question, we compare the "Human-Only" results with the performance of the intervention-based methods. The single operator experiment results show that on both the Threading and Coffee Machine tasks, our method outperforms the "Human-Only" baseline by significant margins ($87.3\%$ vs. $76.7\%$ on Threading, $99.3\%$ vs. $74.0$ on Coffee Machine). This trend holds true even for the intermediate rounds, showing that intervention-based data collection can produce higher quality policies with fewer human-annotated samples. We also see that other intervention-based baselines do not necessarily improve upon the human-only performance - both HG-DAgger and Ours (no balancing) reach roughly the same level of performance as the human-only baseline on the Threading task, and only the Ours (no balancing) baseline is able to outperform the human-only baseline on the Coffee Machine task ($92.0\%$ vs. $74.0\%$). Only our method is able to consistently leverage intervention data to outperform the human-only baseline.

\textbf{Does using our method outperform baselines that learn from intervention data?} Table X compares the per-round results of our method against the other intervention-based baselines on data collected by a single operator. The results demonstrate that our method outperforms both the HG-DAgger baseline and the variant of our method without balancing consistently in each round across both the Threading and Coffee Machine tasks. 

\textbf{Is there value in doing more rounds of intervention data collection compared to collecting the same amount of data in a single round?} For each intervention-based method, we compare the performance of 3 rounds of intervention-based data collection against collecting an equivalent amount of intervention data in a single round. Interestingly enough, doing more rounds of intervention data does not necessarily improve performance over simply collecting a large amount of data in a single round. For our method, we observe no difference in average performance on the Threading task (both are $87.3\%$) and a $7\%$ increase ($99.3\%$ vs. $92.7\%$) on the Coffee Machine task - which are marginal improvements from choosing to carry out multiple rounds. Some of our baselines actually benefit more from doing a single large round of intervention data collection - such as Ours (no balancing) on Threading ($74.7\%$ vs. $84.7\%$) and HG-DAgger on Coffee Machine ($70.0\%$ vs. $92.7\%$). This suggests that scale of data might matter more than swapping out the base policy more frequently. 

\textbf{Does our method outperform other methods on datasets that were collected using their intermediate policies?} To answer this question, we take the final aggregated datasets for each intervention-based method, and train policies on this dataset for all models. The results in Table X demonstrate that our method consistently outperforms other baselines on their collected datasets and can reach a level of performance close to its own collected dataset. This suggests that other baselines do not fail purely due to lower quality data or worse base policies at each iteration, but due to the way they leverage the data. The HG-DAgger baseline does not use implicit policy regularization because it discards the on-policy samples, and Ours (nb) does not appropriately re-weight the intervention samples to reinforce bottleneck-traversing behaviors. Both components are important to achieve the best performance across all datasets. We also emphasize that our method consistently outperforms the "Human-Only" baseline on the datasets collected by other methods, even in cases where the method would not. Comparing across columns in Table X, it is also clear that dataset quality does matter for final performance across all methods - using the dataset collected by our method generally improves the final performance of all methods compare to the HG-DAgger datasets.

\textbf{Do the results hold across different human operators?} TODO: put some suggested takeaways here.

% NOTE: all tables generated using https://www.tablesgenerator.com/latex_tables#

% TABLE - single operator results
\begin{table}[t!]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on Single Operator Datasets:} NOTE: This is reporting MAX over 3 seeds. Each method started with the same human demonstration dataset, base policy, and round 1 intervention dataset. However, the data in round 2 and 3 are different because of the different base policies used for collection. All collection was conducted with 1 human operator.}
\begin{tabular}{cccc}
\hline
\multicolumn{4}{|c|}{Threading}                                                                                       \\ \hline
\multicolumn{1}{|c|}{Model}      & Round 1              & Round 2              & \multicolumn{1}{c|}{Final}           \\ \hline
\multicolumn{1}{|c|}{Base}       & -                    & -                    & \multicolumn{1}{c|}{$58.0 \pm 9.17$} \\
\multicolumn{1}{|c|}{Human-Only} & -                    & -                    & \multicolumn{1}{c|}{$76.7 \pm 2.31$} \\
\multicolumn{1}{|c|}{HG-DAgger}  & $57.3 \pm 9.45$      & $62.7 \pm 5.03$      & \multicolumn{1}{c|}{$75.3 \pm 8.08$} \\
\multicolumn{1}{|c|}{Ours (nb)}  & $76.0 \pm 6.93$      & $72.0 \pm 3.46$      & \multicolumn{1}{c|}{$74.7 \pm 1.15$} \\
\multicolumn{1}{|c|}{Ours}       & $\mathbf{84.0 \pm 5.30}$      & $\mathbf{90.7 \pm 3.06}$      & \multicolumn{1}{c|}{$\mathbf{87.3 \pm 5.03}$} \\ \hline
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                 \\ \hline
\multicolumn{4}{|c|}{Coffee Machine}                                                                                  \\ \hline
\multicolumn{1}{|c|}{Model}      & Round 1              & Round 2              & \multicolumn{1}{c|}{Final}           \\ \hline
\multicolumn{1}{|c|}{Base}       & -                    & -                    & \multicolumn{1}{c|}{$52.0 \pm 3.46$} \\
\multicolumn{1}{|c|}{Human-Only} & -                    & -                    & \multicolumn{1}{c|}{$74.0 \pm 4.00$} \\
\multicolumn{1}{|c|}{HG-DAgger}  & $59.3 \pm 16.7$      & $64.7 \pm 13.3$      & \multicolumn{1}{c|}{$70.0 \pm 12.0$} \\
\multicolumn{1}{|c|}{Ours (nb)}  & $82.0 \pm 6.0$       & $89.3 \pm 5.03$      & \multicolumn{1}{c|}{$92.0 \pm 5.30$} \\
\multicolumn{1}{|c|}{Ours}       & $\mathbf{90.0 \pm 0.00}$      & $\mathbf{90.0 \pm 4.0}$       & \multicolumn{1}{c|}{$\mathbf{99.3 \pm 1.15}$} \\ \hline
\end{tabular}
\label{table:single}
\end{table}


\begin{table}[t!]
\centering
\caption{\textbf{Comparison of Single vs. Iterative Intervention Data Collection:} TODO}
\begin{tabular}{ccc}
\hline
\multicolumn{3}{|c|}{Threading}                                                                    \\ \hline
\multicolumn{1}{|c|}{Model}     & Single Collection    & \multicolumn{1}{c|}{Iterative Collection} \\
\multicolumn{1}{|c|}{HG-DAgger} & $79.3 \pm 2.31$      & \multicolumn{1}{c|}{$75.3 \pm 8.08$}      \\
\multicolumn{1}{|c|}{Ours (nb)} & $84.7 \pm 1.15$      & \multicolumn{1}{c|}{$74.7 \pm 1.15$}      \\
\multicolumn{1}{|c|}{Ours}      & $\mathbf{87.3 \pm 2.31}$      & \multicolumn{1}{c|}{$\mathbf{87.3 \pm 5.03}$}      \\ \hline
\multicolumn{1}{l}{}            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                      \\ \hline
\multicolumn{3}{|c|}{Coffee Machine}                                                               \\ \hline
\multicolumn{1}{|c|}{Model}     & Single Collection    & \multicolumn{1}{c|}{Iterative Collection} \\
\multicolumn{1}{|c|}{HG-DAgger} & $\mathbf{92.7 \pm 5.03}$      & \multicolumn{1}{c|}{$70.0 \pm 12.0$}      \\
\multicolumn{1}{|c|}{Ours (nb)} & $88.7 \pm 5.77$      & \multicolumn{1}{c|}{$92.0 \pm 5.30$}      \\
\multicolumn{1}{|c|}{Ours}      & $\mathbf{92.7 \pm 5.77}$      & \multicolumn{1}{c|}{$\mathbf{99.3 \pm 1.15}$}      \\ \hline
\end{tabular}
\label{table:single_large}
\end{table}



% TABLE - single operator cross
\begin{table}[t!]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on each other's final datasets:} Filled out table. TODO: caption here with takeaways.}
\begin{tabular}{cccc}
                                & \multicolumn{3}{c}{Threading}                                                                       \\ \cline{2-4} 
\multicolumn{1}{c|}{}           & \multicolumn{3}{c|}{Final Dataset}                                                                  \\ \hline
\multicolumn{1}{|c|}{Model}     & HG-DAgger                & Ours (nb)                & \multicolumn{1}{c|}{Ours}                     \\ \hline
\multicolumn{1}{|c|}{HG-DAgger} & $75.3 \pm 8.08$          & $72.0 \pm 5.30$          & \multicolumn{1}{c|}{$81.3 \pm 4.16$}          \\
\multicolumn{1}{|c|}{Ours (nb)} & $80.0 \pm 1.36$          & $74.7 \pm 1.15$          & \multicolumn{1}{c|}{$86.0 \pm 4.0$}           \\
\multicolumn{1}{|c|}{Ours}      & $\mathbf{87.3 \pm 6.43}$ & $\mathbf{84.7 \pm 6.43}$ & \multicolumn{1}{c|}{$\mathbf{87.3 \pm 5.03}$} \\ \hline
\multicolumn{1}{l}{}            & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}                          \\
                                & \multicolumn{3}{c}{Coffee Machine}                                                                  \\ \cline{2-4} 
\multicolumn{1}{c|}{}           & \multicolumn{3}{c|}{Final Dataset}                                                                  \\ \hline
\multicolumn{1}{|c|}{Model}     & HG-DAgger                & Ours (nb)                & \multicolumn{1}{c|}{Ours}                     \\ \hline
\multicolumn{1}{|c|}{HG-DAgger} & $70.0 \pm 12.0$          & $\mathbf{96.7 \pm 3.06}$ & \multicolumn{1}{c|}{$91.3 \pm 7.57$}          \\
\multicolumn{1}{|c|}{Ours (nb)} & $79.3 \pm 4.62$          & $92.0 \pm 5.30$          & \multicolumn{1}{c|}{$89.3 \pm 6.11$}          \\
\multicolumn{1}{|c|}{Ours}      & $\mathbf{91.3 \pm 6.11}$ & $\mathbf{96.7 \pm 3.06}$ & \multicolumn{1}{c|}{$\mathbf{99.3 \pm 1.15}$} \\ \hline
\end{tabular}
\label{table:single_cross}
% \vspace{-8pt}
\end{table}


% TABLE - multi operator
% NOTE: operator 2 is danfei and 3 is josiah
\begin{table}[t]
\centering
\caption{\textbf{Consistency across multiple human operators}}
\begin{tabular}{|l|c|ccc|}
\hline
\multicolumn{5}{|c|}{Coffee Machine}                                                                                         \\ \hline
\multicolumn{1}{|c|}{Operator} & Model      & Round 1                  & Round 2                  & Final                    \\ \hline
                               & Human-Only & -                        & -                        & $74.0 \pm 4.00$          \\
\multicolumn{1}{|c|}{1}        & HG-DAgger  & $59.3 \pm 16.7$          & $64.7 \pm 13.3$          & $70.0 \pm 12.0$          \\
                               & Ours       & $\mathbf{90.0 \pm 0.00}$ & $\mathbf{90.0 \pm 4.0}$  & $\mathbf{99.3 \pm 1.15}$ \\ \hline
                               & Human-Only & -                        & -                        & $56.0 \pm 3.46$          \\
\multicolumn{1}{|c|}{2}        & HG-DAgger  & $66.7 \pm 11.4$          & $\mathbf{74.0 \pm 10.0}$ & $62.7 \pm 2.31$          \\
                               & Ours       & $\mathbf{74.0 \pm 2.00}$ & $69.3 \pm 13.0$          & $\mathbf{81.3 \pm 3.06}$ \\ \hline
                               & Human-Only & -                        & -                        & $64.7 \pm 1.15$          \\
\multicolumn{1}{|c|}{3}        & HG-DAgger  & $\mathbf{84.7 \pm 5.03}$ & $74.7 \pm 1.15$          & $76.0 \pm 11.1$          \\
                               & Ours       & $74.7 \pm 8.08$          & $\mathbf{79.3 \pm 6.11}$ & $\mathbf{82.0 \pm 5.30}$ \\ \hline
                               & Human-Only & -                        & -                        & 64.9                     \\
\multicolumn{1}{|c|}{Avg}      & HG-DAgger  & 70.2                     & 71.1                     & 69.6                     \\
                               & Ours       & $\mathbf{79.6}$          & $\mathbf{79.5}$          & $\mathbf{87.5}$          \\ \hline
\end{tabular}
\label{table:multi}
% \vspace{-8pt}
\end{table}


% TABLE - multi cross
\begin{table}[t!]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on each other's final datasets for multiple human operators}}
\begin{tabular}{cccc}
\multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}           & \multicolumn{2}{c}{Coffee Machine}                              \\ \cline{3-4} 
\multicolumn{1}{l}{}                     & \multicolumn{1}{c|}{}          & \multicolumn{2}{c|}{Final Dataset}                              \\ \hline
\multicolumn{1}{|l|}{Operator}           & \multicolumn{1}{c|}{Model}     & HG-DAgger                & \multicolumn{1}{c|}{Ours}            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{1}} & \multicolumn{1}{c|}{HG-DAgger} & $70.0 \pm 12.0$          & \multicolumn{1}{c|}{$91.3 \pm 7.57$} \\
\multicolumn{1}{|c|}{}                   & \multicolumn{1}{c|}{Ours}      & $\mathbf{91.3 \pm 6.11}$ & \multicolumn{1}{c|}{$\mathbf{99.3 \pm 1.15}$} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{2}} & \multicolumn{1}{c|}{HG-DAgger} & $62.7 \pm 2.31$          & \multicolumn{1}{c|}{$59.3 \pm 1.15$} \\
\multicolumn{1}{|c|}{}                   & \multicolumn{1}{c|}{Ours}      & $\mathbf{84.7 \pm 3.05}$ & \multicolumn{1}{c|}{$\mathbf{81.3 \pm 3.06}$} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{3}} & \multicolumn{1}{c|}{HG-DAgger} & $76.0 \pm 11.1$          & \multicolumn{1}{c|}{$64.0 \pm 9.17$} \\
\multicolumn{1}{|c|}{}                   & \multicolumn{1}{c|}{Ours}      & $\mathbf{80.7 \pm 6.11}$ & \multicolumn{1}{c|}{$\mathbf{82.0 \pm 5.30}$} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Avg}} & \multicolumn{1}{c|}{HG-DAgger} & 69.6                     & \multicolumn{1}{c|}{71.5}            \\
\multicolumn{1}{|c|}{}                   & \multicolumn{1}{c|}{Ours}      & $\mathbf{85.6}$          & \multicolumn{1}{c|}{$\mathbf{87.5}$} \\ \hline
\end{tabular}
\label{table:multi_cross}
\vspace{-8pt}
\end{table}

==> 5-experiment.tex <==
\section{Experimental Setup}
\label{sec:exp}

\subsection{Tasks}
All tasks were designed using MuJoCo~\cite{todorov2012mujoco} and the robosuite framework~\cite{robosuite2020}. The workspace consists of a Sawyer robotic arm in front of a table. The arm is controlled using an Operational Space Controller~\cite{khatib1987unified} and unless otherwise mentioned, the action space for the agent is a 7-dimensional vector where the first 3 coordinates are the desired delta position from the current end effector position, the next 3 coordinates encode the desired delta rotation from the current end effector rotation, and the final coordinate controls the opening and closing of the gripper fingers. The delta rotation is encoded in axis-angle form, where the norm of the 3-vector is the angle, and normalizing the 3-vector produces the axis of the rotation.

% \textbf{Peg-In-Hole}: The robot arm begins each episode with a square peg in its hand, and must insert the peg into a block with a square hole. The location of the block is randomized at the start of each episode. For this task, the robot arm has a reduced 4-dimensional action space that only controls the arm position and gripper - the rotation is held upright. This task is provided as a pedagogical example that contains a single bottleneck region - the insertion of the peg. We designed a closed-form intervention expert for this task, that is able to simulate how a human would intervene and assist the agent, when it fails to insert the peg into the hole.

% \todo{include details of intervention expert when it is finalized}

\textbf{Threading}: At the start of each episode, a wooden rod  and wooden ring are placed on the table. The robot arm must pick up the wooden rod and insert it into the wooden ring. The location of the wooden rod and ring are randomized at the start of each episode. The insertion part of this task is significantly more challenging than the Peg-In-Hole task - insertion requires high precision, and it is easy for the robot arm to unintentionally move the wooden ring if the rod hits the ring. This task contains two bottleneck regions - the grasping of the rod and the insertion into the ring. The observation space consists of the end effector pose, gripper finger positions, and the poses of the wooden rod and ring.

\textbf{Coffee Machine}: At the start of each episode, a coffee pod and a coffee machine are placed on the table. The robot arm must pick up the coffee pod, insert it into the pod holder, and then close the lid of the coffee machine. The location of the coffee pod is randomized at the start of each episode. This task has three bottleneck regions - grasping, insertion, and closing. Both the pod grasping and insertion must be precise, as small errors will cause the pod to slip out of the hand, or fail to be inserted into the holder. The closing of the lid also requires extended contact between the lid and the hand, and misalignment in the closing motion would result in the lid staying open. The observation space consists of the end effector pose, gripper finger positions, the poses of the pod and pod holder, the hinge angle of the lid, and binary contact indicators between the pod, pod holder, and gripper fingers.

\subsection{Baselines}

In this section, we list the baselines we compare against and why each is meaningful.

\textbf{Human-Only}: A human operator collects full task demonstrations instead of intervention-based collection. The full trajectories are added to the dataset and policies are trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of leveraging intervention-based data collection tailored to policy failures over soliciting full task demonstrations that are agnostic to how policies fail on the task.

\textbf{HG-Dagger}: As in~\cite{kelly2019hg, ablett2020fighting} at each round of intervention data collection, only the samples where the user was intervening are added to the dataset, while the policy samples are discarded. Policies are trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of keeping policy samples to train the policy for the next round.

\textbf{Ours (no balancing)}: At each round of intervention data collection, all samples are added to the dataset, including the policy samples, and the next policy is trained with normal BC over the aggregated data. Comparing against this baseline highlights the value of using balanced sampling in our method to reweight the data distribution.

\textbf{Ours}: Same as Ours (no balancing), but aggregates the policy samples and intervention samples into separate datasets and uses balanced sampling to re-weight the data distribution during learning.

\subsection{Experiment Details}

We conducted two data collection studies to demonstrate the utility of our system and our method for learning from intervention data. In the first, a single operator collected multiple sequences of datasets on the Threading and Coffee Machine tasks. In the second, multiple human operators collected datasets on the Coffee Machine tasks. 

% which amounted to 7205 samples for the Threading task, and 6620 samples for the Coffee Machine task
Each operator started with an initial dataset that consisted of 30 demonstrations for each task, and a base policy that was trained on each initial dataset. Then, for each intervention-based method, the operator performed 3 additional rounds of data collection. During each round, the operator collected trajectories until the number of intervention data samples reached roughly $33\%$ of the initial dataset samples. We only counted intervention data samples so that all methods would be able to receive the same number of human-annotated samples at each round, regardless of the quality of the base policy, and to be consistent with prior work~\cite{kelly2019hg}. After each round, the base policy for the next round was obtained by training for 2000 epochs on the aggregated dataset and taking the final checkpoint, in order to model the realistic setting where policy evaluation is expensive. Note that the Round 1 datasets will be the same for all methods but Round 2 and Round 3 will be different because data collection occurs on separate base policies.

For the "Human-Only" baseline, each operator collected a single dataset of human demonstration trajectories that consisted of roughly the same number of samples as the initial dataset. For the "Single" variants of the intervention-based methods, an operator performed a single round of intervention data collection on the initial base policy, gathering roughly the same number of intervention samples as the initial dataset. This dataset is shared for all methods for the same reason that the Round 1 datasets are the same.

All policies were Recurrent Neural Networks - 2-layer LSTMs with hidden dimension 100, trained on a sequence length of 10 using Adam optimizers~\cite{kingma2014adam}. At test-time, the hidden state was refreshed every 10 timesteps. To evaluate each method, policies were saved after every 50 epochs and evaluated with 50 rollouts for each checkpoint. All success rates presented in each table reflect the maximum average success rate obtained by each training run over all model checkpoints, for 3 training runs with different seeds. We emphasize that the procedure of training multiple runs, checkpointing, and evaluating policies was performed after data collection for all runs was complete - the numbers played no role in selecting base policies for the next round.

\subsection{Experiments}

\textbf{Does data collected using our intervention-based system improve task performance more than an equivalent amount of human-only demonstration samples?} To answer this question, we compare the "Human-Only" results with the performance of the intervention-based methods. The single operator experiment results show that on both the Threading and Coffee Machine tasks, our method outperforms the "Human-Only" baseline by significant margins ($87.3\%$ vs. $76.7\%$ on Threading, $99.3\%$ vs. $74.0$ on Coffee Machine). This trend holds true even for the intermediate rounds, showing that intervention-based data collection can produce higher quality policies with fewer human-annotated samples. We also see that other intervention-based baselines do not necessarily improve upon the human-only performance - both HG-DAgger and Ours (no balancing) reach roughly the same level of performance as the human-only baseline on the Threading task, and only the Ours (no balancing) baseline is able to outperform the human-only baseline on the Coffee Machine task ($92.0\%$ vs. $74.0\%$). Only our method is able to consistently leverage intervention data to outperform the human-only baseline.

\textbf{Does using our method outperform baselines that learn from intervention data?} Yes - look at table.

\textbf{Is there value in doing more rounds of intervention data collection compared to collecting the same amount of data in a single round?} For each intervention-based method, we compare the performance of 3 rounds of intervention-based data collection against collecting an equivalent amount of intervention data in a single round. Interestingly enough, doing more rounds of intervention data does not necessarily improve performance over simply collecting a large amount of data in a single round. For our method, we observe no difference in average performance on the Threading task (both are $87.3\%$) and a $7\%$ increase ($99.3\%$ vs. $92.7\%$) on the Coffee Machine task - which are marginal improvements from choosing to carry out multiple rounds. Some of our baselines actually benefit more from doing a single large round of intervention data collection - such as Ours (no balancing) on Threading ($74.7\%$ vs. $84.7\%$) and HG-DAgger on Coffee Machine ($70.0\%$ vs. $92.7\%$). This suggests that scale of data might matter more than swapping out the base policy more frequently. 

\textbf{Does our method outperform other baselines on datasets that were collected using their intermediate policies?}
Key takeaways - dataset quality can matter - both Ours (nb) and Ours uniformly improve results across all methods. Our method also consistently performs the best across other datasets, showing that it is an effective way to learn from interventions. It also shows that in cases where the baseline methods were not able to outperform human-only, our method can do so using the same set of data (so method is critical).

\textbf{Do the results hold across different human operators?} TODO: put some suggested takeaways here.

% \begin{itemize}
%     \item (Peg-In-Hole) Comprehensive Comparison with closed-form Intervention Expert
%     \begin{itemize}
%         \item Compare all Interactive Policy Learning Methods on a sequence of datasets they collect.
%         \item Key Results: show that as we increase the amount of suboptimality in the intervention expert, our method outperforms other baselines.
%         \item Requires \textbf{3 * number of baselines} automated data collections - should be cheap. 
%     \end{itemize}
%     \item (Threading / Coffee) Comparison of Interactive Policy Learning Methods and Human-Only data
%     \begin{itemize}
%         \item For each baseline, with 1 human, collect 3 rounds of intervention data using the same base policy. Also collect an equivalent amount of additional human-only data and add it to the base dataset used to train the base policy. Optionally also add full on-policy trajectories from the base policy to the human-only dataset to compare with (to give it an equivalent amount of data and be more fair).
%         \item Key Results: show that (1) intervention datasets result in better performance than human-only data, given the same number of \textit{human} samples and (2) our method outperforms other baselines on these challenging tasks.
%         \item Requires \textbf{2 tasks * 3 rounds * num baselines + 2 base datasets}.
%     \end{itemize}
%     \item (Threading / Coffee) Off-Policy Interactive Policy Learning - learning from another policy's failures
%     \begin{itemize}
%         \item take seqeunce of datasets collected by each method, and train on same data with a different method.
%         \item Key Result: Our method can leverage data collected by other base policies / methods and improve the results there too, despite witnessing "off-policy" failures. Rationale is that failure coverage is more important for these domains than specific instance of failure.
%         \item No additional data required.
%     \end{itemize}
%     \item (Threading / Coffee) Consistency across Multiple Humans
%     \begin{itemize}
%         \item For each human and the same fixed base policy, collect 3 rounds of intervention datasets using our method at each round, and an additional equivalent amount of data collected purely from the human.
%         \item Key Result: Show that our method produces better results than the human-only data, across all humans.
%         \item Requires \textbf{3 humans * (2 tasks * 3 rounds + 2 base datasets)}. So each person collects 8 datasets in total. For each additional baseline, each human would need to collect 6 more datasets.
%     \end{itemize}
%     %  NOTE: skipping this experiment
%     % \item (Threading / Coffee) Consistency across different base policies
%     % \begin{itemize}
%     %     \item In all the above experiments, we held the base policy constant. We can show that our method is consistent across 3 different base policies.
%     %     \item TODO: is this valuable? It will be a relatively expensive experiment to run. We could run it on Peg-In-Hole but then it wouldn't be as interesting.
%     %     \item Requires \textbf{2 tasks * (3 base policies * 3 rounds + 3 base datasets)}. More if we compare against other baselines.
%     % \end{itemize}
% \end{itemize}

==> 6-results.tex <==
\section{Results}
\label{sec:results}

% \begin{table}[t]
% \centering
% \caption{\textbf{Comparison of Intervention-Based Learning Methods on Peg-In-Hole:} TODO - compare peg-in-hole with varied suboptimality in intervention expert, and show that ours is better.}
% \begin{tabular}{|c|cccc|}
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Peg-In-Hole} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% HG-DAgger & 100\% & 0.0\% & 100\% & 50.0\%    \\
% Ours (no balancing) & 50.0\% & 100\% & 0.0\% & 50.0\%   \\
% Ours & 77.2\% & 68.9\% & 31.1\% & 100\% \\ \hline
% \end{tabular}
% \label{table:sim}
% \vspace{-8pt}
% \end{table}


\begin{table}[t]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on Threading and Coffee Machine:} NOTE: This is reporting MAX over 3 seeds. Each method started with the same human demonstration dataset, base policy, and round 1 intervention dataset. However, the data in round 2 and 3 are different because of the different base policies used for collection. All collection was conducted with 1 human operator.}
\begin{tabular}{|c|cccc|}
\hline
{\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Threading} \\ \hline
Model & Base & Round 1 & Round 2 & Final \\ \hline
Human-Only & $58.0 \pm 9.17$ & - & - & $76.7 \pm 2.31$    \\
HG-DAgger (Single) & $58.0 \pm 9.17$ & - & - & $79.3 \pm 2.31$    \\
Ours (nb) (Single) & $58.0 \pm 9.17$ & - & - & $84.7 \pm 1.15$    \\
Ours (Single) & $58.0 \pm 9.17$ & - & - & $87.3 \pm 2.31$    \\
HG-DAgger & $58.0 \pm 9.17$ & $57.3 \pm 9.45$ & $62.7 \pm 5.03$ & $75.3 \pm 8.08$    \\
Ours (nb) & $58.0 \pm 9.17$ & $76.0 \pm 6.93$ & $72.0 \pm 3.46$ & $74.7 \pm 1.15$   \\
Ours & $58.0 \pm 9.17$ & $84.0 \pm 5.30$ & $90.7 \pm 3.06$ & $87.3 \pm 5.03$ \\ \hline
\hline
\hline
{\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine} \\ \hline
Model & Base & Round 1 & Round 2 & Final \\ \hline
Human-Only & $52.0 \pm 3.46$ & - & - & $74.0 \pm 4.00$    \\
HG-DAgger (Single) & $52.0 \pm 3.46$ & - & - & $92.7 \pm 5.03$    \\
Ours (nb) (Single) & $52.0 \pm 3.46$ & - & - & $88.7 \pm 5.77$    \\
Ours (Single) & $52.0 \pm 3.46$ & - & - & $92.7 \pm 5.77$    \\
HG-DAgger & $52.0 \pm 3.46$ & $59.3 \pm 16.7$ & $64.7 \pm 13.3$ & $70.0 \pm 12.0$    \\
Ours (nb) & $52.0 \pm 3.46$ & $82.0 \pm 6.0$ & $89.3 \pm 5.03$ & $92.0 \pm 5.30$   \\
Ours & $52.0 \pm 3.46$ & $90.0 \pm 0.00$ & $90.0 \pm 4.0$ & $99.3 \pm 1.15$ \\ \hline

\end{tabular}
\label{table:sim}
\vspace{-8pt}
\end{table}


% \begin{table}[t]
% \centering
% \caption{\textbf{Comparison of Intervention-Based Learning Methods on Threading and Coffee Machine:} TODO - fill in results for each model and each round of intervention (and base). Each method started with the same human demonstration dataset, base policy, and round 1 intervention dataset. However, the data in round 2 and 3 are different because of the different base policies used for collection. All collection was conducted with 1 human operator.}
% \begin{tabular}{|c|cccc|}
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Threading (no GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 34.8\% & - & - & 47.2\%    \\
% HG-DAgger (Single) & 34.8\% & - & - & 41.6\%    \\
% Ours (no balancing) (Single) & 34.8\% & - & - & 70.8\%    \\
% % Ours (variant) (Single) & 34.8\% & - & - & 65.2\%    \\
% Ours (Single) & 34.8\% & - & - & 55.0\%    \\
% HG-DAgger & 34.8\% & 23.2\% & 34.6\% & 63.0\%    \\
% Ours (no balancing) & 34.8\% & 49.6\% & 44.0\% & 62.2\%   \\
% % Ours (variant) & 34.8\% & 48.0\% & 69.8\% & 64.4\%  \\
% Ours & 34.8\% & 59.4\% & 63.6\% & 57.4\% \\ \hline
% \hline
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine (no GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 24.2\% & - & - & 51.0\%    \\
% HG-DAgger (Single) & 24.2\% & - & - & 46.0\%    \\
% Ours (no balancing) (Single) & 24.2\% & - & - & 62.8\%    \\
% % Ours (variant) (Single) & 24.2\% & - & - & 75.4\%    \\
% Ours (Single) & 24.2\% & - & - & 78.8\%    \\
% HG-DAgger & 24.2\% & 34.8\% & 34.4\% & 29.8\%    \\
% Ours (no balancing) & 24.2\% & 59.4\% & 80.0\% & 55.4\%   \\
% % Ours (variant) & 24.2\% & 53.0\% & 85.4\% & 72.4\%   \\
% Ours & 24.2\% & 67.2\% & 63.4\% & 84.6\% \\ \hline
% \hline
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine (GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 29.8\% & - & - & 61.4\%    \\
% HG-DAgger (Single) & 29.8\% & - & - & 66.2\%    \\
% Ours (no balancing) (Single) & 29.8\% & - & - & 60.2\%    \\
% % Ours (variant) (Single) & 29.8\% & - & - & 68.4\%    \\
% Ours (Single) & 29.8\% & - & - & 67.6\%    \\
% HG-DAgger & 29.8\% & 59.6\% & 55.2\% & 69.2\%    \\
% Ours (no balancing) & 29.8\% & 47.6\% & 55.4\% & 74.4\%   \\
% % Ours (variant) & 29.8\% & 54.8\% & 55.4\% & 79.6\%   \\
% Ours & 29.8\% & 67.2\% & 77.4\% & 83.4\% \\ \hline

% \end{tabular}
% \label{table:sim}
% \vspace{-8pt}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{\textbf{Comparison of Intervention-Based Learning Methods on Threading and Coffee Machine:} VARIANT: use best average consecutive epoch performance (over 5 checkpoints, 50 epochs apart).}
% \begin{tabular}{|c|cccc|}
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Threading (no GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 41.4\% & - & - & 64.8\%    \\
% HG-DAgger (Single) & 41.4\% & - & - & 50.4\%    \\
% Ours (no balancing) (Single) & 41.4\% & - & - & 77.6\%    \\
% % Ours (variant) (Single) & 41.4\% & - & - & 77.4\%    \\
% Ours (Single) & 41.4\% & - & - & 66.4\%    \\
% HG-DAgger & 41.4\% & 32.6\% & 47.2\% & 74.4\%    \\
% Ours (no balancing) & 41.4\% & 62.4\% & 60.2\% & 67.2\%   \\
% % Ours (variant) & 41.4\% & 60.4\% & 75.2\% & 69.0\%  \\
% Ours & 41.4\% & 75.6\% & 80.0\% & 71.2\% \\ \hline
% \hline
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine (no GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 30.8\% & - & - & 64.2\%    \\
% HG-DAgger (Single) & 30.8\% & - & - & 76.6\%    \\
% Ours (no balancing) (Single) & 30.8\% & - & - & 65.8\%    \\
% % Ours (variant) (Single) &30.82\% & - & - & 86.6\%    \\
% Ours (Single) & 30.8\% & - & - & 78.8\%    \\
% HG-DAgger & 30.8\% & 34.8\% & 34.4\% & 37.6\%    \\
% Ours (no balancing) & 30.8\% & 59.4\% & 80.0\% & 71.4\%   \\
% % Ours (variant) & 30.8\% & 65.0\% & 86.0\% & 78.4\%   \\
% Ours & 30.8\% & 67.2\% & 70.0\% & 86.4\% \\ \hline
% \hline
% \hline
% {\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine (GMM)} \\ \hline
% Model & Base & Round 1 & Round 2 & Final \\ \hline
% Human-Only & 29.8\% & - & - & 67.4\%    \\
% HG-DAgger (Single) & 29.8\% & - & - & 66.8\%    \\
% Ours (no balancing) (Single) & 29.8\% & - & - & 66.8\%    \\
% % Ours (variant) (Single) & 29.8\% & - & - & 75.8\%    \\
% Ours (Single) & 29.8\% & - & - & 72.8\%    \\
% HG-DAgger & 29.8\% & 59.6\% & 58.4\% & 72.4\%    \\
% Ours (no balancing) & 29.8\% & 55.2\% & 55.4\% & 75.8\%   \\
% % Ours (variant) & 29.8\% & 60.0\% & 62.2\% & 83.2\%   \\
% Ours & 29.8\% & 73.4\% & 78.2\% & 84.8\% \\ \hline

% \end{tabular}
% \label{table:sim}
% \vspace{-8pt}
% \end{table}

\begin{table}[t]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on each other's final datasets:} Filled out table. TODO: caption here with takeaways.}
\begin{tabular}{|c|ccc|}
\hline
{\color[HTML]{000000} Threading} & \multicolumn{3}{c|}{Final Dataset} \\ \hline
Model & HG-DAgger & Ours (nb) & Ours \\ \hline
HG-DAgger & $75.3 \pm 8.08$ & $72.0 \pm 5.30$ & $81.3 \pm 4.16$  \\
Ours (nb) & $80.0 \pm 1.36$ & $74.7 \pm 1.15$ & $86.0 \pm 4.0$  \\
Ours & $87.3 \pm 6.43$ & $84.7 \pm 6.43$ & $87.3 \pm 5.03$ \\ \hline
\hline
\hline
{\color[HTML]{000000} Coffee Machine} & \multicolumn{3}{c|}{Final Dataset} \\ \hline
Model & HG-DAgger & Ours (nb) & Ours \\ \hline
HG-DAgger & $70.0 \pm 12.0$ & $96.7 \pm 3.06$ & $91.3 \pm 7.57$   \\
Ours (nb) & $79.3 \pm 4.62$ & $92.0 \pm 5.30$ & $89.3 \pm 6.11$  \\
Ours & $91.3 \pm 6.11$ & $96.7 \pm 3.06$ & $99.3 \pm 1.15$ \\ \hline
\end{tabular}
\label{table:sim}
\vspace{-8pt}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Consistency across multiple human operators:} TODO - fill in results for each model and each round of intervention (and base). Each method started with the same human demonstration dataset, base policy, and round 1 intervention dataset. However, the data in round 2 and 3 are different because of the different base policies used for collection.}
\begin{tabular}{|c|cccc|}
\hline
{\color[HTML]{000000} Task} & \multicolumn{4}{c|}{Coffee Machine} \\ \hline
Model & Base & Round 1 & Round 2 & Final \\ \hline
Human-Only (Danfei) & $52.0 \pm 3.46$ & - & - & $56.0 \pm 3.46$    \\
HG-DAgger (Danfei) & $52.0 \pm 3.46$ & $66.7 \pm 11.4$ & $74.0 \pm 10.0$ & $62.7 \pm 2.31$    \\
Ours (Danfei) & $52.0 \pm 3.46$ & $74.0 \pm 2.00$ & $69.3 \pm 13.0$ & $81.3 \pm 3.06$ \\ 
\hline
Human-Only (Josiah) & $52.0 \pm 3.46$ & - & - & $64.7 \pm 1.15$    \\
HG-DAgger (Josiah) & $52.0 \pm 3.46$ & $84.7 \pm 5.03$ & $74.7 \pm 1.15$ & $76.0 \pm 11.1$    \\
Ours (Josiah) & $52.0 \pm 3.46$ & $74.7 \pm 8.08$ & $79.3 \pm 6.11$ & $82.0 \pm 5.30$ \\ 
\hline
Human-Only (Albert) & $52.0 \pm 3.46$ & - & - & $52.7 \pm 4.16$    \\
HG-DAgger (Albert) & $52.0 \pm 3.46$ & $52.0 \pm 2.23$ & $81.3 \pm 14.0$ & $84.0 \pm 8.72$    \\
Ours (Albert) & $52.0 \pm 3.46$ & $66.7 \pm 3.06$ & $64.0 \pm 18.3$ & $54.0 \pm 5.30$ \\ 
\hline
% HG-DAgger (All operators) & - & - & - & -    \\
% Ours (All operators) & - & - & - & - \\ \hline
\end{tabular}
\label{table:sim}
\vspace{-8pt}
\end{table}



\begin{table}[t]
\centering
\caption{\textbf{Comparison of Intervention-Based Learning Methods on each other's final datasets:} Filled out table. TODO: caption here with takeaways.}
\begin{tabular}{|c|cc|}
\hline
{\color[HTML]{000000} Coffee Machine} & \multicolumn{2}{c|}{Final Dataset} \\ \hline
Model & HG-DAgger & Ours \\ \hline
HG-DAgger (Danfei) & $62.7 \pm 2.31$ & $59.3 \pm 1.15$ \\
Ours (Danfei) & $84.7 \pm 3.05$ & $81.3 \pm 3.06$ \\ \hline
HG-DAgger (Josiah) & $76.0 \pm 11.1$ & $64.0 \pm 9.17$ \\
Ours (Josiah) & $80.7 \pm 6.11$ & $82.0 \pm 5.30$ \\ \hline
HG-DAgger (Albert) & $84.0 \pm 8.72$ & $81.3 \pm 8.08$ \\
Ours (Albert) & $78.7 \pm 11.0$ & $54.0 \pm 5.30$ \\ \hline
\end{tabular}
\label{table:sim}
\vspace{-8pt}
\end{table}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/full_placeholder.png}
%     \caption{\textbf{Qualitative Examples of Mistakes and Corrections} We showcase some examples of mistakes than can occur in the absence of a human operator as well as corrections demonstrated by the human interventions across different human operators for both the Threading and Coffee Machine tasks.}
%     \label{fig:corrections}
%     % \vspace{0.5mm}
%     \vspace{-15pt}
% \end{figure*}
